A unified stochastic approximation framework for learning in games

We develop a flexible stochastic approximation framework for analyzing the long-run behavior of learning in games (both continuous and finite). The proposed analysis template incorporates a wide array of popular learning algorithms, including gradient-based methods, the exponential/multiplicative weights algorithm for learning in finite games, optimistic and bandit variants of the above, etc. In addition to providing an integrated view of these algorithms, our framework further allows us to obtain several new convergence results, both asymptotic and in finite time, in both continuous and finite games. Specifically, we provide a range of criteria for identifying classes of Nash equilibria and sets of action profiles that are attracting with high probability, and we also introduce the notion of coherence, a game-theoretic property that includes strict and sharp equilibria, and which leads to convergence in finite time. Importantly, our analysis applies to both oracle-based and bandit, payoff-based methods - that is, when players only observe their realized payoffs.

==> Body/Algorithms.tex <==
%----------------------------------------------------------------------
%%% ALGORITHMS
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


We now proceed to describe a representative range of methods for learning in games.
Depending on the information available to the players, we classify the algorithms under study as \emph{oracle-based} or \emph{payoff-based};
% (\cf \cref{sec:oracle,sec:bandit} respectively).
our presentation scheme in the rest of this section reflects this taxonomy.


%----------------------------------------------------------------------
%% Feedback
%----------------------------------------------------------------------
\subsection{Oracle-based methods}
\label{sec:oracle}

%The common denominator of the algorithms we present below is that they are all iterative, closed-loop methods with a ``black-box'' model for the game being played.
%More precisely, as the learning process unfolds, we assume that each player can query a \acdef{SFO} that provides information about the player's payoff function at the selected action profile.

The commmon denominator of the algorithms we discuss below is that players have access to a ``black-box''  feedback mechanism \textendash\ a \acdef{SFO} \textendash\ that returns an estimate of their individual payoff gradients at their chosen action profile.%
\footnote{Methods that require full, ``white-box'' knowledge of the game's payoff functions are not treated here.}
Formally, when queried at $\point\in\points$, an \ac{SFO} outputs a random vector
%$\orcl = (\orcl_{\play})_{\play\in\players}$
%$\orcl = (\orcl_{1},\dotsc,\orcl_{\nPlayers})$
of the form
\begin{align}
\label{eq:SFO}
\tag{SFO}
\orcl(\point;\seed)
	&= \vecfield(\point)
	+ \err(\point;\seed),
\end{align}
where
$\seed$ is a random variable taking values in some measurable space $\seeds$
and
$\err(\point;\seed)$ is an umbrella error term capturing all sources of uncertainty in the model.
%(observational noise, minibatch selection, etc.).

In practice, \eqref{eq:SFO} is queried repeatedly at a sequence of action profiles $\curr\in\points$, $\run=\running$, possibly with a different random seed $\curr[\seed]$ at each time.%
\footnote{In some cases, the index set may be enlarged to include all positive half-integers ($\run = \halfrunning$).}
To keep track of this sequence of events, we will view $\curr$ as a stochastic process on some complete probability space $\probspace$, and we will write $\curr[\filter] \defeq \filter(\init,\dotsc,\curr) \subseteq \filter$ for the \emph{history of play} up to \textendash\ and including \textendash\ stage $\run$.
Accordingly, since the randomness entering the oracle is triggered only \emph{after} each player has selected an action, we will posit throughout that $\curr[\seed]$ is $\next[\filter]$-measurable \textendash\ though not necessarily $\curr[\filter]$-measurable.
For concreteness, we will also assume that the noise in \eqref{eq:SFO} is zero-mean and bounded in $L^{\qexp}$ for some $\qexp\geq2$, \ie
\begin{equation}
\label{eq:oracle}
\exof{\err(\point;\curr[\seed]) \given \curr[\filter]}
	= 0
	\quad
	\text{and}
	\quad
\exof{\dnorm{\err(\point;\curr[\seed])}^{\qexp} \given \curr[\filter]}
	\leq \sdev^{\qexp}
%	\;\;
%	\text{for some $\sdev\geq0$}.
\end{equation}
for some $\sdev\geq0$ and all $\point\in\points$.
In particular (and in a slight abuse of notation), the case $\qexp=\infty$ above refers to the case when the noise is bounded \ac{wp1}, that is, $\dnorm{\err(\point;\curr[\seed])} \leq \sdev$ \as.

\smallskip

We are now in a position to introduce the array of oracle-based methods under study.
For simplicity, we present some of these policies in an unconstrained setting;
this is only done to lighten the notation.

\smallskip

%----------------------------------------------------------------------
\begin{algo}[\Acl{SGA}]
\label{alg:SGA}

Perhaps the most basic iterative policy for multi-agent online learning is the standard (individual) gradient ascent method
\begin{align}
%\next
%	&= \curr - \curr[\step] \vecfield(\curr)
%\shortintertext{or, more explicitly, for each player $\play\in\players$:}
\label{eq:SGA}
\tag{SGA}
\state_{\play,\run+1}
	&= \state_{\play,\run} + \curr[\step] \orcl_{\play}(\curr;\curr[\seed]).
\end{align}
Informally, \eqref{eq:SGA} implies that all players are simultaneously taking a stochastic gradient step with step-size $\curr[\step] > 0$.
%(we discuss this parameter later).
From a loss minimization viewpoint, \eqref{eq:SGA} is a multi-agent analogue of the standard \acl{SGD} algorithm;
analogously, in min-max games, \eqref{eq:SGA} boils down to the Arrow\textendash Hurwicz method \citep{AHU58}.
\endenv
\end{algo}
%----------------------------------------------------------------------

In the sequel, all gradients will be assumed stochastic, so we will not highlight this explicitly.

%----------------------------------------------------------------------
\begin{algo}[\Acl{seqGA}]
\label{alg:seqGA}
A common variant of \eqref{eq:SGA} is when players update their actions turn-by-turn instead of simultaneously.
This results in the \acli{seqGA} policy
\begin{equation}
\label{eq:seqGA}
\tag{\acs{seqGA}}
\begin{aligned}
\state_{\play,\run+1}
	&= \state_{\play,\run}
		+ \curr[\step] \orcl_{\play}(\dotsc,\state_{\play-1,\run+1},\state_{\play,\run},\state_{\play+1,\run},\dotsc;\curr[\seed]).
\end{aligned}
\end{equation}
%for all $\play = 1,\dotsc,\nPlayers$.
Formally, the only difference between \eqref{eq:SGA} and \eqref{eq:seqGA} lies in the oracle query at the update step:
instead of computing all gradients at $\curr$, each individual gradient in \eqref{eq:seqGA} is computed sequentially after each player has locked in an action.
This variant is widely used in \acp{GAN} \cite{GPAM+14,DISZ18,HMC21}.
\endenv
\end{algo}
%----------------------------------------------------------------------


%----------------------------------------------------------------------
\begin{algo}[\Acl{EG}]
\label{alg:EG}
Going a step further from \eqref{eq:SGA}, the \acdef{EG} algorithm of \citet{Kor76} is based on the following principle:
starting at some ``base'' state $\curr$, the players first take a gradient step to an interim, ``leading'' state $\lead$;
subsequently, to anticipate their payoff landscape, they update the base state $\curr$ with gradient information from $\lead$ instead of $\curr$.
% and the process repeats.
Formally, this leads to the policy
\begin{equation}
\label{eq:EG}
\tag{\acs{EG}}
\begin{aligned}
\state_{\play,\run+1/2}
	&= \state_{\play,\run} + \curr[\step] \orcl_{\play}(\curr;\curr[\seed]),
	\\
\state_{\play,\run+1}
	&= \state_{\play,\run} + \curr[\step] \orcl_{\play}(\lead;\lead[\seed]).
\end{aligned}
\end{equation}
For applications of this method to \acp{GAN} and robust reinforcement learning, see \cite{MLZF+19,kamalaruban2020robust}.
\endenv
\end{algo}
%----------------------------------------------------------------------


%----------------------------------------------------------------------
\begin{algo}[\Acl{OG}]
\label{alg:OG}
A computational drawback of \eqref{eq:EG} is that it requires two oracle queries per update
\textendash\ and hence, more overhead per iteration.
One way to overcome this hurdle is to reuse past gradient information in the hope that it provides a good enough approximation of the present;
this leads to the \acli{OG} policy
\begin{equation}
\label{eq:OG}
\tag{\acs{OG}}
\begin{aligned}
\state_{\play,\run+1/2}
	&= \state_{\play,\run} + \curr[\step] \orcl_{\play}(\beforelead;\prev[\seed]),
	\\
\state_{\play,\run+1}
	&= \state_{\play,\run} + \curr[\step] \orcl_{\play}(\lead;\curr[\seed]).
\end{aligned}
\end{equation}
The ``gradient reuse'' idea in \eqref{eq:OG} dates back at least to \citet{Pop80}, and it has resurfaced several times in the literature since then, \cf \cite{RS13-NIPS,DISZ18,HIMM19} and references therein.
To simplify our presentation, we will assume in the sequel that the method is run with an \ac{SFO} satisfying \eqref{eq:oracle} with $\qexp = \infty$.
\endenv
\end{algo}
%----------------------------------------------------------------------


The next method concerns learning in mixed extensions of finite games.
%(\cf \cref{ex:mixed} in \cref{sec:prelims}).


%----------------------------------------------------------------------
\begin{algo}[\Acl{EW}]
\label{alg:EW}
Let $\game = \mixgame$ be the mixed extension of a finite game $\fingamefull$ as per \cref{ex:mixed}.
In this setting, the players' learning process typically unfolds as follows:
at each stage $\run=\running$, every player selects a mixed strategy $\state_{\play,\run} \in \simplex(\pures_{\play})$ and draws a pure strategy $\pure_{\play,\run} \in \pures_{\play}$ according to $\state_{\play,\run}$.
Then, depending on the amount of information available to the players, we have the following oracle models:
\begin{subequations}
\label{eq:SFO-finite}
\begin{enumerate}
\item
\emph{Full information feedback:}
in this case, players observe their \emph{mixed} payoff vectors, \ie
\begin{align}
\label{eq:SFO-finite-full}
\orcl_{\play}(\curr;\curr[\pure])
	&= \payv_{\play}(\state_{\play,\run};\state_{-\play,\run}).
\shortintertext{%
\item
\emph{Realization-based feedback:}
here, players instead observe their \emph{pure} payoff vectors, \ie
} % end intertext
\label{eq:SFO-finite-realized}
\orcl_{\play}(\curr;\curr[\pure])
	&= \payv_{\play}(\pure_{\play,\run};\pure_{-\play,\run}).
\end{align}
\end{enumerate}
\end{subequations}
In both models, the seed of the oracle is the action profile $\curr[\pure]$ chosen by the players at stage $\run$:
the oracle \eqref{eq:SFO-finite-full} is deterministic, while the oracle \eqref{eq:SFO-finite-realized} is stochastic and satisfies \eqref{eq:oracle} with $\qexp=\infty$.

In this context, one of the most widely used methods is the \acli{EW} algorithm
\begin{align}
\label{eq:EW}
\tag{\acs{EW}}
\begin{split}
\dstate_{\play,\run+1}
	&= \dstate_{\play,\run} + \curr[\step] \orcl_{\play}(\curr;\curr[\pure])
	\\
\state_{\play,\run+1}
	&= \logit_{\play}(\dstate_{\play,\run+1})
\end{split}
\shortintertext{where $\logit_{\play}$ denotes the ``logit choice'' map}
\logit_{\play}(\dpoint_{\play})
	&= \frac
		{(\exp(\dpoint_{\play\pure_{\play}}))_{\pure_{\play}\in\pures_{\play}}}
		{\sum_{\pure_{\play}\in\pures_{\play}} \exp(\dpoint_{\play\pure_{\play}})}
\end{align}
and $\orcl_{\play}$ is given by \eqref{eq:SFO-finite-full} or \eqref{eq:SFO-finite-realized} depending on the information available to the players.
%In words, \eqref{eq:EW} selects a pure strategy with probability that is exponential in its cumulative payoff up to the current stage.
This method has a very long history in online learning and game theory;
for an appetizer, see \citet{Vov90,LW94} and \citet{ACBFS95}.
%\footnote{In the literature, a closely related variant of \eqref{eq:EW} is referred to as the \acli{MWU}, \cf \citet{AHK12}.
%%The two algorithms are closely related but not equivalent;
%To avoid any confusion, we will only use the terminology ``\acl{EW}''.}
\endenv
\end{algo}
%----------------------------------------------------------------------

The last oracle-based method we present concerns games with general action spaces.

%----------------------------------------------------------------------
\begin{algo}[\Acl{MP}]
\label{alg:MP}
An important generalization of the \acl{EG} method (\cref{alg:EG}) is the \acli{MP} algorithm \cite{Nem04,JNT11}, which we define here as follows:
\begin{equation}
\label{eq:MP}
\tag{\acs{MP}}
\begin{alignedat}{3}
\lead[\dstate]
	&= \curr[\dstate] + \curr[\step] \orcl(\curr;\curr[\seed])
	&\qquad
\next[\dstate]
	&= \curr[\dstate] + \curr[\step] \orcl(\lead;\lead[\seed])
	\\
\lead
	&= \mirror(\lead[\dstate])
	&\qquad
\next
	&= \mirror(\next[\dstate]).
\end{alignedat}
\end{equation}
In the above, $\mirror\from\dspace\to\points$ denotes the namesake \emph{mirror map} of the method, as it is used to ``mirror'' the extra-gradient chain $\curr[\dstate] \to \lead[\dstate] \to \next[\dstate] \in \dspace$ into feasible action profiles $\curr \to \lead \to \next \in \points$.
As an example, in the Euclidean unconstrained case ($\points=\pspace$), the identity map $\mirror(\dpoint) = \dpoint$ yields the \acl{EG} algorithm (\cref{alg:EG});
as another example, in finite games, letting $\mirror = \logit$ gives the so-called ``simplex setup'' of \eqref{eq:MP}.
We provide more details on this construction in \cref{sec:framework} below.
\endenv
\end{algo}
%----------------------------------------------------------------------


%----------------------------------------------------------------------
%% Payoff-based methods
%----------------------------------------------------------------------
\subsection{Payoff-based methods}
\label{sec:bandit}

In many applications to machine learning and data science, unbiased gradient estimates can be obtained by making a partial pass over the problem's training data;
in such cases, players can query \eqref{eq:SFO} directly.
By contrast, in applications to auctions, online advertising and networks, players may only be able to observe their realized payoffs.
In this case, gradients must be somehow reconstructed from payoff-based observations, as players cannot perform direct queries to \eqref{eq:SFO}.
In view of this distinction,
we describe below a range of \emph{payoff-based} policies where players do not have access to an oracle, but must infer gradient information indirectly.


%----------------------------------------------------------------------
\begin{algo}[\Acl{SPSA}]
\label{alg:SPSA}
\acused{SPSA}
%When gradients are not readily available (either because they are too costly to compute or because the game's payoff functions are not known in closed form), the players must emulate a gradient signal based on their incurred payoffs.
A straightforward way of reconstructing gradients from zeroth-order feedback is via the \acli{SPSA} framework of \citet{Spa92}.
In the unconstrained case ($\points=\pspace$), the relevant update step is:
\begin{equation}
\label{eq:SPSA}
\tag{SPSA}
\begin{aligned}
\query_{\play,\run}
	&= \state_{\play,\run} + \curr[\mix] \unitvar_{\play,\run},
	\\
\state_{\play,\run+1}
	&= \state_{\play,\run}
		+ \curr[\step] (\pay_{\play}(\curr[\query]) / \curr[\mix]) \,  \unitvar_{\play,\run}.
\end{aligned}
\end{equation}
In \eqref{eq:SPSA}, each player's ``query state'' $\query_{\play,\run}$, $\play=1,\dotsc,\nPlayers$, is a perturbation of the ``base state'' $\state_{\play,\run}$ by a step of magnitude $\curr[\mix]>0$ along a random direction $\unitvar_{\play,\run}$ drawn from the ensemble of signed basis vectors
$\bvecs_{\play} \defeq \{(\pm\bvec_{1},\dotsc,\pm\bvec_{\vdim_{\play}})\}$.
Importantly, \eqref{eq:SPSA} can be seen as a special case of \eqref{eq:SGA} with the ``virtual'' oracle $\orcl_{\play}(\point;\unitvec) = (\vdim_{\play}/\mix) \, \pay_{\play}(\point+\mix\unitvec) \, \unitvec_{\play}$ where each $\unitvec_{\play}$ is drawn uniformly at random from $\bvecs_{\play}$.
As we discuss in \cref{sec:examples}, this estimator is biased, so it does not satisfy \eqref{eq:oracle}; see also \cref{tab:algorithms}.
%a bias of $\bigoh(\curr[\mix])$ and a variance of $\bigoh(1/\curr[\mix]^{2})$.

We should stress here that the above formulation of \eqref{eq:SPSA} is tailored to unconstrained problems.
In this case, to ensure that the resulting gradient estimator remains bounded, it is customary to include an indicator of the form $\oneof{\norm{\curr[\query]} \leq \curr[R]}$ for some suitably chosen sequence $\curr[R]\to\infty$ \cite{Spa92}.
This would lead to the same analysis but at the cost of heavier notation;
thus, to avoid overloading the presentation, we will assume instead that the players' payoff functions are bounded when discussing \eqref{eq:SPSA}.

Of course, in games with compact action spaces (as per \cref{sec:prelims}) this last point is moot.
In that case however, certain book-keeping adjustments are required to ensure that $\curr[\query] \in \points$ for all $\run$.
For a detailed discussion of how to adapt \eqref{eq:SPSA} in the presence of constraints, we refer the reader to \citet{BLM18} who show that the relevant entries of \cref{tab:algorithms} apply verbatim when $\points$ is compact.
\endenv
\end{algo}
%----------------------------------------------------------------------


%----------------------------------------------------------------------
\begin{algo}[\Acl{DGA}]
\label{alg:DGA}
\acused{DGA}
An alternative approach to \eqref{eq:SPSA} is the ``explore-then-update'', two-point sampling approach of \citet{BBF20}.
Specifically, \citet{BBF20} focused on games with $\points_{\play} = [0,\infty)$ for all $\play\in\players$ and introduced the \acli{DGA} policy
\begin{equation}
\label{eq:DGA}
\tag{DGA}
\begin{aligned}
\state_{\play,\run+1/2}
	&= \state_{\play,\run} + (1/\run) \unitvar_{\play,\run},
	\\
\state_{\play,\run+1}
	&= \state_{\play,\run} \bracks{1 + (\pay_{\play}(\lead) - \pay_{\play}(\curr)) \unitvar_{\play,\run}},
\end{aligned}
\end{equation}
where, at each $\run=\running$, the ``exploration direction'' $\unitvar_{\play,\run}$ is sampled uniformly at random from $\{\pm 1\}$.
In words, \eqref{eq:DGA} is a two-stage process in which players first ``explore'' their individual payoff functions at a nearby state, and then use this information to estimate their individual payoff gradients and update their base state.
\endenv
\end{algo}
%----------------------------------------------------------------------


%----------------------------------------------------------------------
\begin{algo}[The \acs{EXP3} algorithm]
\label{alg:EXP3}
In our final example, we return to finite games, and we focus on the ``bandit'' case where players can only observe the payoffs of the pure strategies that they actually played.
%Here, an additional difficulty is that players can only observe the payoffs of their \emph{pure} strategies, not their mixed ones.
%%formally, this means that the game's mixed payoff functions $\pay_{\play}(\point)$ can only be sampled at pure strategy profiles, not mixed ones.
%Because of this, continuous estimators like \eqref{eq:SPSA} and \eqref{eq:DGA} cannot be used in finite games:
%if the queried state is a mixed strategy, the associated mixed payoff will be, in general, unobservable.
In this setting, it is common to employ the \acli{IWE}
\begin{equation}
\label{eq:IWE}
\tag{IWE}
\orcl_{\play\pure_{\play}}(\curr[\query];\curr[\purequery])
	= \frac
		{\oneof{\purequery_{\play,\run} = \pure_{\play}}}
		{\query_{\play\pure_{\play},\run}}
			\pay_{\play}(\purequery_{\play,\run};\purequery_{-\play,\run})
	\qquad
	\text{for all $\pure_{\play}\in\pures_{\play}$, $\play\in\players$},
\end{equation}
where each player $\play\in\players$ draws an action $\purequery_{\play,\run}$ from $\pures_{\play}$ according to a mixed strategy $\query_{\play,\run}  \in \simplex(\pures_{\play})$, \cf \cite{CHM17-NIPS,GVM21,LS20} and references therein.
Then, plugging \eqref{eq:IWE} into \eqref{eq:EW}, we obtain the method known as \acdef{EXP3}, viz.
\begin{align}
\label{eq:EXP3}
\tag{EXP3}
\begin{split}
\dstate_{\play,\run+1}
	&=\dstate_{\play,\run} + \curr[\step] \orcl_{\play}(\curr[\query];\curr[\purequery]),
	\\
\state_{\play,\run+1}
	&= \logit_{\play}(\dstate_{\play,\run+1}),
\end{split}
\shortintertext{where the sampling strategy of the $\play$-th player at stage $\run$ is given by}
\label{eq:explore}
\query_{\play,\run}
	&= (1-\curr[\mix]) \state_{\play,\run} + \curr[\mix] \unif(\pures_{\play}).
\end{align}
In the above, $\curr[\mix] \geq 0$ is an ``explicit exploration'' parameter that determines the mixing between $\state_{\play,\run}$ and the uniform distribution $\unif(\pures_{\play})$ on $\pures_{\play}$.
%The role of $\curr[\mix]$ is discussed in detail in the sequel;
%For a detailed treatise on \eqref{eq:EXP3}, see \citet{LS20}.
\endenv
\end{algo}
%----------------------------------------------------------------------


In closing this section, we note that we can also ``mix'n'match'' the above algorithms to form new ones:
for instance,
%coupling the \acs{SPSA} estimator of \cref{alg:SPSA} with the a mirror map as in \cref{alg:MP} leads to the \acl{BMD} algorithm of \citet{BLM18};
incorporating the gradient reuse step of \eqref{eq:OG} in the simplex setup for \eqref{eq:MP} yields the \acf{OMW} method of \citet{DP19}.
%running \eqref{eq:EW} with gradient input on minimization problems gives the \ac{EGD} algorithm of \citet{BecTeb03};
%etc.
In the sections to come, we provide a synthetic view and analysis of all these policies.
